A Distance-based Framework for Gaussian Processes over Probability Distributions

Gaussian processes constitute a very powerful and well-understood method for non-parametric regression and classification. In the classical framework, the training data consists of deterministic vector-valued inputs and the corresponding (noisy) measurements whose joint distribution is assumed to be Gaussian. In many practical applications, however, the inputs are either noisy, i.e., each input is a vector-valued sample from an unknown probability distribution, or the probability distributions are the inputs. In this paper, we address Gaussian process regression with inputs given in form of probability distributions and propose a framework that is based on distances between such inputs. To this end, we review different admissible distance measures and provide a numerical example that demonstrates our framework.

==> Sections/03_LCD.tex <==
%
As outlined above, 

==> Sections/10_mCvMD.tex <==
%
In this section, we briefly introduce the modified Cram\'{e}r--von Mises distance. Historically, the mCvMD was developed for deterministic sampling of continuous densities~\cite{Hanebeck_2008,Hanebeck_2009}. To this end, it was necessary to generalize the multivariate cumulative distribution in order to be able to compare continuous and Dirac densities. The result was the Localized Cumulative Distribution (LCD) that we describe in the next section before presenting the mCvMD.

%-----------------------------------------------------------------------------------------
\subsection{Localized Cumulative Distribution}

The LCD of the multivariate pdf $p(\nvec{x})\in\IR^\dimx$ is defined according to
%
\begin{align*}
	F(\nvec{m},\nvec{b})
		&=
		\int\limits_{\IR^n} p(\nvec{x}) \kappa(\nvec{x},\nvec{m},\nvec{b}) \d\nvec{x}\ ,
\end{align*}
%
where $\kappa(\cdot,\cdot,\cdot)$ is a suitable kernel with location parameter $\nvec{m}\in\IR^\dimx$ and expansion parameter $\nvec{b}>0$ (component-wise). Often, the kernel is chosen to be isotropic which yields a positive scalar expansion parameter $b$.  Suitable kernels reported in literature include the (non-isotropic) uniform distribution, the unit disk, and Radial Basis Functions (RBFs). We propose to use (isotropic) RBFs
%
\begin{align}
	\kappa(\nvec{x},\nvec{m},b)
		&=
		\exp\klammer{-\frac{1}{2}\frac{(\nvec{x}-\nvec{m})\tr(\nvec{x}-\nvec{m})}{b^2}}
	\label{eq:LCD}
\end{align}
%
because for these kernels it was shown that the LCD of any arbitrary pdf is unique~\cite{Gilitschenski_2015}.

%-----------------------------------------------------------------------------------------
\subsection{Distance Measure}

With the above definition of the LCD, we can formulate the distance between the two densities $p_i(\nvec{x})\in\IR^\dimx$ and $p_j(\nvec{x})\in\IR^\dimx$ as follows. Let $F_i(\nvec{m},b)\in\IR^{\dimx+1}$ and $F_j(\nvec{m},b)\in\IR^{\dimx+1}$ denote the LCDs of $p_i(\nvec{x})$ and $p_j(\nvec{x})$, respectively. Then, the mCvMD between the densities can be computed according to
%
\begin{align}
	d(p_i(\nvec{x}),p_j(\nvec{x}))
		&=\hspace{-1mm}
		\int\limits_{\IR^n} \int\limits_{\IR_+} \hspace{-1mm} w(b) \klammer{F_i(\nvec{m},b)-F_j(\nvec{m},b)}^2\hspace{-1mm} \d b\d\nvec{m}\ ,
	\label{eq:mCvMD}
\end{align}
%
where $w(b)$ is a suitable weighting function that is necessary in order to ensure the convergence of the integral if the used kernel functions have infinite support.

Of course, the evaluation of the integrals in~\eqref{eq:LCD} and~\eqref{eq:mCvMD} is not trivial. However, there exist efficient solutions for many practically interesting cases such as Gaussians, Gaussian mixtures, or Dirac densities (see, e.g., \cite{Gilitschenski_2013,Gilitschenski_2014,Hanebeck_2015}).
